To Augment or Not to Augment? A Comparative Study on Text Augmentation Techniques for Low-Resource NLP

Data-hungry deep neural networks have established themselves as the standard for many NLP tasks including the traditional sequence tagging ones. Despite their state-of-the-art performance on high-resource languages, they still fall behind of their statistical counter-parts in low-resource scenarios. One methodology to counter attack this problem is text augmentation, i.e., generating new synthetic training data points from existing data. Although NLP has recently witnessed a load of textual augmentation techniques, the field still lacks a systematic performance analysis on a diverse set of languages and sequence tagging tasks. To fill this gap, we investigate three categories of text augmentation methodologies which perform changes on the syntax (e.g., cropping sub-sentences), token (e.g., random word insertion) and character (e.g., character swapping) levels. We systematically compare them on part-of-speech tagging, dependency parsing and semantic role labeling for a diverse set of language families using various models including the architectures that rely on pretrained multilingual contextualized language models such as mBERT. Augmentation most significantly improves dependency parsing, followed by part-of-speech tagging and semantic role labeling. We find the experimented techniques to be effective on morphologically rich languages in general rather than analytic languages such as Vietnamese. Our results suggest that the augmentation techniques can further improve over strong baselines based on mBERT. We identify the character-level methods as the most consistent performers, while synonym replacement and syntactic augmenters provide inconsistent improvements. Finally, we discuss that the results most heavily depend on the task, language pair, and the model type.

==> aug_param.tex <==
Apart from the augmentation technique specific settings (e.g., labels of interest for cropping), some of the parameters are common to most methods and may have a substantial impact on the success of the methods.  

\paragraph{Ratio:} This parameter is used to calculate the number of new sentences to be generated from one original sentence. To ensure that more sentences are generated from longer sentences, it is simply calculated as $ratio*original sentence length$, i.e., for a sentence of length 10, only 1 extra sentence will be produced by augmentation. It is only used for ortographic methods since syntactic methods are constrained in other ways (e.g., number of tokens that share morphological features and dependency labels). The values we experiment with are as follows: 0.1, 0.2, 0.3 and 0.4.

\paragraph{Probability:} This determines the probability of a token-level augmentation, i.e., the ratio of the augmented tokens to sentence length. For word insertion, deletion and all character-based methods (CI, CD, CSU, CSW, CA), it can be interpreted as the ratio of tokens that undergo a change to all tokens; while for word swapping operation, it refers to the ratio of swapped token pairs to all tokens. Moreover, it determines the number of characters to which the augmentation are applied in case of character-level augmentation. Similar to ratio, we experiment with the values: 0.1, 0.2, 0.3 and 0.4. For the syntactic methods crop and rotate, probability is associated with the operation dynamics, i.e., when the operation probability is set to 0.2\%, the expected number of additional sentences produced via cropping would be $\#LOI/5$, where $\#LOI$ indirectly refers to the number of valid subtrees for the operation.  

\paragraph{Max Sentences:} In case of considerably long sentences or substantial number of available candidates, the number of augmented sentences can grow rapidly. This sometimes causes an undesired level of noise in the training data. To avoid this, the number of maximum sentences, a.k.a., sentence threshold parameter, is commonly used. We experiment with 5 and 10 as the threshold values. 


% Maybe move to experimental details
%As the cropping technique is capable of generating $\#LOI$ additional sentences, while the rotation can produce up to $(\#LOI+1)!$ additional data points, we limit the number of \#LOIs. Following \citet{SahinS18}, we \textit{only} consider the dependency relations that attach subjects and objects to predicates as LOIs; and ignore other adverbial dependency links involving predicates. In addition, we use language-specific dependency labels to detect the predicates that consist of multiple tokens such as multiword expressions, light verbs, copulas or morphological derivations. Similar to \citet{SahinS18}, we keep the augmentation non-recursive, i.e., we only reorder the first level of flexible subtrees, hence the flexible chunks inside these subtrees are kept fixed. We further the limit the number of rotations to 3, as suggested in \cite{SahinS18}, and perform each operation with a predefined probability. %For instance, when the operation probability is set to 25\%, the expected number of additional sentences produced via cropping would be  $\#LOI/4$.

==> eval.tex <==
For all the tasks, we use the standard evaluation measures commonly used in literature. Accuracy is used to evaluate POS tagging results. To evaluate SRL results, we used the official CoNLL-09 evaluation script on the official test split. The script calculates the macro-average F1 scores for the semantic roles available in the data. For dependency parsing, we use the Labeled Attachment Score (LAS).

==> neural_param.tex <==
%We use orthogonal initialization for all network components. The model is optimized via stochastic gradient descent with initial learning rate as 1. We trained the models for 50 epochs, and used early stopping when the results on development set do not improve after 3 epochs. The same hyperparameters are used to train various SRL models on original and augmented training datasets. ~\todo{Write the main settings} The embedding size for characters are chosen as 200 and we used one layer bidirectional LSTMs for both word embedding composition and argument labeling layer.. We experiment with different number of layers: one and two bi-LSTM network/s both for the word composition and labeling layers.

\paragraph{POS Tagging and SRL} 
We used uniform initialization for all network components. The model is optimized via stochastic gradient descent with initial learning rate as 1. Gradients above $2$ are clipped. We trained the models for 50 epochs, and decrease the learning rate by half when the results on development set do not improve after 3 epochs. The embedding size for characters as well as hidden size of intermediate layers are chosen as 128. Batch size is set to 8 due to small training set. Number of bi-LSTM layers of all bi-LSTM components are left as a parameter and the values 1 and 2 are used in the experiments.

\paragraph{Dependency Parsing}
We used the default settings of the uuparser~\cite{KiperwasserG16,delhoneux17arc}\footnote{Available at \url{https://github.com/UppsalaNLP/uuparser}}. Similar to POS tagging, embedding sizes are set to 128, and the training is performed for 100 epochs.  


